Working Memory Capacity of ChatGPT: An Empirical Study

Working memory is a critical aspect of both human intelligence and artificial intelligence, serving as a workspace for the temporary storage and manipulation of information. In this paper, we systematically assess the working memory capacity of ChatGPT, a large language model developed by OpenAI, by examining its performance in verbal and spatial n-back tasks under various conditions. Our experiments reveal that ChatGPT has a working memory capacity limit strikingly similar to that of humans. Furthermore, we investigate the impact of different instruction strategies on ChatGPT's performance and observe that the fundamental patterns of a capacity limit persist. From our empirical findings, we propose that n-back tasks may serve as tools for benchmarking the working memory capacity of large language models and hold potential for informing future efforts aimed at enhancing AI working memory.

==> 8-rebuttal.tex <==
\newcommand{\rone}[1][]{\textcolor{cyan}{R1}\xspace}
\newcommand{\rthree}[1][]{\textcolor{red}{R3}\xspace}
\newcommand{\rfour}[1][]{\textcolor{blue}{R4}\xspace}
\newcommand{\rfive}[1][]{\textcolor{orange}{R5}\xspace}


\noindent\textbf{\rone, Q1. [Whether the n-back task can reflect the working memory ability of LLMs]} In the context of our paper, the definition of “working memory” comes from human studies (Baddeley 1992), where both n-back tasks and working memory span tasks (Conway et al. 2005) have been used to measure working memory capacity. However, n-back tasks are arguably the gold standard because we can manipulate the working memory load in the task (Kane and Engle 2002). Also, n-back tasks have good construct validity and correlate with other WM measures (Jaeggi et al. 2010).

% \smallskip 

\noindent\textbf{\rone, Q2. [Did not see the comparison of ChatGPT's working memory capacity limit to that of humans]} We mentioned in the introduction that “typical human performance drops significantly when n = 3 (Klatzky et al. 2008; Amon and Bertenthal 2018), which can be defined as the working memory capacity limit of an average human”.

% \smallskip 

\noindent\textbf{\rone, Q3. [Unconvincing to evaluate the working memory ability of LLMs through an n-back task]} To the best of our knowledge, this work is the first to empirically define and evaluate the “working memory capacity” of LLMs. Research has shown that working memory capacity is a strong correlate of human intelligence in general, and our comparisons of multiple LLMs on the n-back task confirmed that their performance is consistent with their overall intelligence as measured by more classical benchmarks (Chang et al. 2023).

% \smallskip 

\noindent\textbf{\rone, Q4. [Working memory capacity of LLMs seems to be intrinsic, but this doesn’t seem to be the case with humans]} Human working memory capacity limit is intrinsic (Cowan 2001), and that’s exactly the starting point of this work – to test if LLMs have a similar capacity limit.

% \smallskip 

\noindent\textbf{\rthree, Q1. [How Figure 2 would change if the verbal task + noise is considered]} Human research has suggested a strong influence of interference on n-back task performance (Gaspar 2016; Ni and Ma 2021), therefore we would expect comparable declines in task performance in this scenario.

% \smallskip 

\noindent\textbf{\rthree, Q2. [Why 8 match trials and 16 nonmatch trials]} The ratio of match and nonmatch trials is based on the convention in human studies (Szmalec et al. 2011).

% \noindent\textbf{\rthree,Q3. [Describe the metrics]} Hit rate: the rate at which targets are correctly identified. False alarm rate: the rate at which non-targets are incorrectly identified. Accuracy: the overall correctness, whether the stimulus is a target or a non-target. Detection sensitivity (d'): the difference between the z-scores of the hit rate and the false alarm rate.
% \smallskip 

\noindent\textbf{\rthree, Q4. [Why Verbal with Feedback leads to comparable or worse results]} We found literature that suggests immediate feedback is not always beneficial (Katz et al. 2014) - immediate feedback after each trial can be distracting as you are constantly monitoring (and evaluating) your performance.

% \smallskip 

\noindent\textbf{\rthree, Q5. [CoT reasoning seems not to have significantly improved model performance]} The Wilcoxon signed rank test statistics in the Appendix show that CoT reasoning improved the model performance on the 2-back task. Here by “significantly improved” we mean the improvement is “statistically significant”.

% \smallskip 

\noindent\textbf{\rfour, W1\&W2. [Does not provide novel methods to improve the existing methods or solve a new problem]} The review criteria mention that the contributions may be theoretical/methodological/\textbf{empirical}... and that papers \textbf{explore new territory} or \textbf{point out new directions for research} are preferred. Through rigorous empirical testing, our paper for the first time connects the working memory capacity of humans to that of LLMs, which introduces a brand-new problem to the field of LLMs. This is an important contribution towards further understanding the relationship between current approaches in LLMs and mechanisms of human cognition.

% \smallskip 

\noindent\textbf{\rfour, W3. [Not clear if LLMs also have limited memory capacity for real-life tasks]} Working memory capacity is a fundamental aspect of human cognition and is not confined to any specific “real-life tasks”. Like any other cognitive ability, working memory capacity is studied under an operational definition. The n-back task is exactly how working memory capacity is operationalized and it has been proved effective by the literature. Note that what humans do in laboratory tasks is never real-life tasks, but that doesn't render these tasks uninformative about how human cognition works.

% \smallskip 

\noindent\textbf{\rfive, W1. [Introduction and prompt designs takes up a large part]} This work sits at the intersection of AI and cognitive science, which means the introduction of background knowledge from cognitive science is crucial for AI researchers who may not be familiar with this topic. We include prompt designs because the experimental design in our work is nuanced, involving intricate task settings that are critical to understand our experimental innovation.

% \smallskip 

\noindent\textbf{\rfive, W2. [More emphases should be placed on explanations and optimization methods]} Below is our explanation and how we might be able to improve LLMs’ working memory capacity. We hypothesize that the self-attention mechanism in the Transformer architecture is responsible for this phenomenon. The self-attention mechanism computes a weighted sum of input elements, which may lead to a diffusion of information across multiple inputs, making it challenging to maintain and access specific pieces of information as n increases in n-back tasks. One possible way to improve this is to increase the number of attention heads in the architecture. More attention heads can allow the model to focus on different parts of the input sequence concurrently (Wang and Tu 2020). This can be crucial for the n-back task as it requires the model to keep track of information at multiple positions in the sequence.

% \smallskip 

\noindent\textbf{\rfive, Q1. [Explainability to the discovered phenomenon from the perspective of pre-training method or LLM architecture design]} Please refer to our response to \rfive, W2.

% \smallskip 

\noindent\textbf{\rfive, Q2. [Whether the evaluation metrics can be used to fine-tune LLMs on this task]} Just as the goal of most studies on human working memory capacity is not to improve it but to quantify individual differences (Cochrane et al. 2019), here we are proposing that working memory capacity is also an intrinsic property of LLMs that can potentially be used an index of the overall intelligence level of different LLMs, as evidenced by the performance of different LLMs on the n-back task.

% \smallskip 

\noindent\textbf{\rfive, Q3. [Whether it is sufficient to use the n-back tasks to test the LLMs]} Please refer to our response to \rone, {Q1}.

% \smallskip 

\noindent\textbf{\rfive, Q4. [Why the larger grid leads to better performance; the influence of string length in the verbal task]} We speculate that when the grid size is larger, there might be less interference between stimulus inputs across trials so that LLMs can better keep track of the information flow without being confused. This is related to the "sparse coding" nature of the grids. However, in the verbal n-back task, increasing the length of every input would probably make it harder for the model to extract specific strings n steps ago, leading to worse model performance in this scenario.
